Sound, Precise, and Fast Abstract Interpretation with Tristate Numbers

Extended Berkeley Packet Filter (BPF) is a language and run-time system that allows non-superusers to extend the Linux and Windows operating systems by downloading user code into the kernel. To ensure that user code is safe to run in kernel context, BPF relies on a static analyzer that proves properties about the code, such as bounded memory access and the absence of operations that crash. The BPF static analyzer checks safety using abstract interpretation with several abstract domains. Among these, the domain of tnums (tristate numbers) is a key domain used to reason about the bitwise uncertainty in program values. This paper formally specifies the tnum abstract domain and its arithmetic operators. We provide the first proofs of soundness and optimality of the abstract arithmetic operators for tnum addition and subtraction used in the BPF analyzer. Further, we describe a novel sound algorithm for multiplication of tnums that is more precise and efficient (runs 33% faster on average) than the Linux kernel's algorithm. Our tnum multiplication is now merged in the Linux kernel.

==> tex/sec.artifact.tex <==
\section{Artifact}

\urlstyle{tt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

Our artifact \cite{vishwanathan-tnums} provides source code for the algorithms
and experiments mentioned in the paper. We describe how to reproduce and
validate the following claims: (i) soundness of tnum operations using the Z3 SMT
solver, (ii) precision improvements in our tnum multiplication algorithm
compared to existing algorithms (iii) performance improvements in our tnum
multiplication algorithm compared to existing algorithms. We provide scripts to
compile the source code and produce the relevant figures. The artifact is open
source and publicly available. We also provide a prebuilt Docker image
containing the required software dependencies for easier evaluation of the
artifact.

\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
\item {\bf Algorithm: }
\begin{itemize}
\item \ourmul, our new algorithm for multiplication of elements in the
abstract domain of tnums, and existing algorithms \reghermul
\cite{regehr-deriving-abstract-transfer}, and \kernmul (from the Linux
kernel).
\item Other existing algorithms for arithmetic, bitwise, and shift
operations in the tnum abstract domain.
\end{itemize}
\item {\bf Program: } C++, Python3
\item {\bf Compilation: } g++ 7.5.0 or above.
\item {\bf Run-time environment: } The experiments were performed on Ubuntu
18.04 with target x86-64 (which is recommended). They were also confirmed to
work on Ubuntu 20.04.
\item {\bf Hardware: } Modern machines with at least 2.3GHz processors and 8GB
memory should be sufficient.
\item {\bf Metrics: } Soundness, precision, and execution time (total number
of cycles).
\item {\bf Output: } Theorem prover output (sat/unsat); log files containing
precision numbers and cycle count; the numbers visualized using graphs.
\item {\bf Experiment workflow: } See below.
\item {\bf How much disk space required (approximately)?: } Around 2GB (for
the Docker image), or around 10MB for the source code and scripts.
\item {\bf How much time is needed to complete experiments (approximately)?: }
1 hour.
\item {\bf Publicly available?: } Yes.
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access} The artifact can be downloaded from the Zenodo
archive at \url{https://doi.org/10.5281/zenodo.5703630}, or cloned from GitHub
at \url{https://github.com/bpfverif/tnums-cgo22}, or from Docker Hub at
\url{https://hub.docker.com/r/mys35/tnums-cgo22}.

\subsubsection{Software dependencies} The implementation of the algorithms is
written in C. The precision and performance experiments are written in C++ and
depend on the Boost C++ library. The soundness verification is written in
Python3 and needs the z3-solver package. The graph plotting scripts are written
in Python3 and depend on numpy and matplotlib. All the necessary software is
installed in the Docker image.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}
We provide two options for installation of the experiment source code and
scripts: (i) using a prebuilt Docker image with all software dependencies
included, and (ii) manually downloading and installating the software and
dependencies. 

Note that the experiments in the paper were performed without using any
container. One of the four experiments measures execution time, so using the
manual option will produce results more in line with the paper (although the
overall trends should be similar). All the other experiments should produce
similar results with either option.

Generally, we recommend running the experiments on a system with no other
compute or memory intensive applications running in the background, to obtain
results that align better with those in the paper.

\subsubsection{Using Docker image} Install Docker if it is not installed already
by following the documentation at \url{https://docs.docker.com/get-docker/}. You
might need to follow the post installation steps for managing docker as a
non-root user \url{https://docs.docker.com/engine/install/linux-postinstall/}.
Then pull the Docker image and run it with the following command:
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]  
$ docker run -it mys35/tnums-cgo22
\end{lstlisting} 

\subsubsection{Manual installation on Ubuntu 18.04} To run the evaluation
without using Docker, first install the required packages:
% , basicstyle=\ttfamily\footnotesize, breaklines=true
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]  
$ sudo apt update
$ sudo apt install -yq libboost-all-dev \
  build-essential python3 python3-(*pi*)p
$ python3 -m (*pi*)p install --upgrade (*pi*)p
$ python3 -m (*pi*)p install z3-solver numpy matplotlib \
  scipy
\end{lstlisting}
Next, clone the artifact repository:
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm].  
$ git clone \
  https://github.com/bpfverif/tnums-cgo22.git
$ cd tnums-cgo22
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}
The artifact provides scripts to automatically conduct the four experiments:
three from the evaluation section (\Sec{evaluation}) of the main paper, and one
presented in the supplementary material (\Sec{supplement}). In the following
sections, we show how to run each experiment one after the other, how to obtain
the expected results, and how to customize the experiment.

% \begin{itemize}
%   \item \emph{Automated verfication of tnum operations with Z3 (\Sec{evaluation})}
%   \item \emph{Relative precision of \ourmul compared to \kernmul and \reghermul
%   (\Sec{evaluation})}
%   \item \emph{Performance of \kernmul vs \reghermul vs. \ourmul (\Sec{evaluation})}
%   \item \emph{Comparing the precision of \ourmul vs. \kernmul with increasing bitwidth
%   (\Sec{supplement})}
% \end{itemize}

\subsection{Notes}
\label{sec:artifact_notes}
\Para{Copying files from Docker container to host.} Some of the experiments
below produce \code{.png} image files. If using Docker to perform the
evaluation, use the following steps to copy files from the docker container to
your local machine.
\begin{enumerate}
  \item In a new terminal run the following command and copy the container ID
  (yours may be different) for the image \code{mys35/tnums-cgo22}:
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ docker ps -a
CONTAINER ID   IMAGE               ... 
30e20b7c68d7   mys35/tnums-cgo22   ...
\end{lstlisting}
\item Copy the \code{.png} file to your local machine
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ docker cp \
  <container_id>:<source_path> <destination_path>
\end{lstlisting}
\end{enumerate}

\Para{Scripts for constant CPU frequency.}\label{sec:scripts} If using the
manual option for evaluation, we provide two scripts in the \code{scripts}
directory for Intel CPUs which help reduce experimental noise for the
performance experiment: (i) \code{constant_freq.sh}, which fixes the CPU
frequency for \emph{all} cores on your machine at 2.2GHz. (ii)
\code{toggle_hyperthreading.sh} which toggles hyperthreading from on to off (and
vice versa). We recommend you run these scripts with \code{sudo} before running
the experiments. A reboot of your machine should reset to the defaults.

\subsection{Experiments}

\Para{Automated verfication of tnum operations with Z3}
\begin{itemize}
  \item Section: \Sec{eval_z3}
  \item Figure: N/A
  \item Estimated time: 5 minutes
\end{itemize}

For all tnum operations except the multiplication operations, \kernmul and
\ourmul, automated verification is performed with bitvectors (i.e. input tnums)
of width $64$. For multiplication, since the automated verification takes a long
time to complete, we perform automated verification with $8$ bits.

\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ cd verification
$ bash verif.sh
\end{lstlisting}

\emph{Expected Results.} The output should show that all operations are verified
for correctness successfully.

\emph{Experiment customization.} The python script \code{tnum.py} accepts
switches \code{----bitwidth} (the bitvector width) and \code{----op} (the tnum
operation for which the verification is to be performed). Each tnum operation
\code{<op>} is encoded as a first-order logic formula using a Python method with
the name \code{tnum_<op>}, and the corresponding soundness verification
condition is encoded in the method \code{check_tnum_<op>}, where \code{<op>} is
\code{add, sub, rshift,} \etc It is easy to add new tnum operations for
verification by following the examples of the existing operations.

\Para{Relative precision of \ourmul compared to \kernmul and \reghermul}
\begin{itemize}
  \item Section: \Sec{eval_precision}
  \item Figure: \ref{fig-rel-pres}
  \item Estimated time: 10 minutes
\end{itemize}
To finish the experiment in a reasonable amount of time, the script compares
precision of the multiplication algorithms for bitvectors of width $8$.
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ cd ../precision-relative
$ bash pres.sh
\end{lstlisting}

\emph{Expected Results.} This experiment will produce a graph called
\code{pres_fig.png} in the same directory. If using Docker, follow the steps
noted above (\Sec{artifact_notes}) to copy the image from the container to the
host machine. For example: 
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ docker cp 30e20b7c68d7:\
  /home/tnums-cgo22/precision-relative/pres_fig.png .
\end{lstlisting}

The figure should be the same as Figure \ref{fig-rel-pres} in the main paper.
The figure indicates that \ourmul is more precise than both \kernmul and
\reghermul.

\emph{Experiment customization.} 
The precision comparison is performed by default for a bitwidth of $8$, this can
be changed by modifying the \code{BITWIDTH} variable in the script
\code{pres.sh}. When compiled with \code{-DKERN_MUL_V_OUR_MUL} and run, the file
\code{precision_relative.cpp} will output the precision comparison between
\kernmul and \ourmul. This works similarly for \code{-DBITWISE_MUL_V_OUR_MUL}.
It is easy to follow the existing examples and add an additional macro guard
(\code{-D...}) which does a different precision comparison. The graphing script
\code{graph_precision_relative.py} can also be similarly extended to accept more
(or fewer) comparision files as input and produce the CDF.

\Para{Performance of \kernmul vs \reghermul vs. \ourmul} 
\begin{itemize}
  \item Section: \Sec{eval_performance}
  \item Figure: \ref{fig-speed}
  \item Estimated time: 20 minutes
\end{itemize}

\emph{Note about reproducing performance results:} To reproduce the results
exactly as shown in the paper, this experiment needs to be run with Turbo Boost
and Hyper-threading disabled, and the CPU has to run at a constant frequency. We
provide scripts for doing this as mentioned in \ref{sec:scripts}. The scripts
only work with the manual evaluation option, and do not work with Docker. Hence,
if you use Docker, it is possible that the results are less aligned with those
in the paper. From our experience running this experiment on Docker (on our
laptops, with Turbo Boost and Hyper-threading still enabled), we found that
\ourmul consistently performs at least as well as the best of the other
variants, with the difference in performance varying across runs.

We highly recommend running this experiment with no other compute-intensive
applications running in the background. Additionally, note that we pin the
experiment thread to a CPU ID $5$. Please change the variable \code{CPU_ID} in
the script \code{perf.sh} according to your architecture, if necessary. To
finish the experiment in a reasonable amount of time, we use 4 million randomly
sampled input tnums to the algorithms, as opposed to 40 million in the main
paper.
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ cd ../performance
$ bash perf.sh
\end{lstlisting}

\emph{Expected Results.} This experiment will produce a graph called
\code{perf_fig.png} in the same directory. If using Docker, follow the steps
noted above (\Sec{artifact_notes}) to copy the image from the container to the
host machine. For example: 
\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ docker cp 30e20b7c68d7:\
  /home/tnums-cgo22/performance/perf_fig.png .
\end{lstlisting}

The figure should be \emph{similar} to Figure \ref{fig-speed} in the main paper.
Using the manual evaluation option after running the required scripts should
give results that align more closely with those in the paper. The results should
indicate that \ourmul is faster on average than \kernmul and \reghermul.

\emph{Experiment customization.} The script allows the following customizations
to its variables: (i) \code{NUM_TNUM_PAIRS}: number of randomly sampled input
tnums, (ii) \code{NUM_TRIALS}: number of trials of the algorithm is run per tnum
pair, (iii) \code{CPU_ID}: the CPU ID to pin the experiment to. The script
passes on these variables to a compiled \code{performance.cpp} as command line
arguments, which outputs the cycle count numbers when run. The file
\code{performance.cpp} and the CDF graphing script \code{graph_performance.py}
can be extended similarly as the previous experiment.

\Para{Comparing the precision of \ourmul vs. \kernmul with increasing
  bitwidth} 
\begin{itemize}
\item Section: \Sec{supplement} (supplementary material)
\item Table: \ref{table:muls_precision_increasing_bitwidth}
\item Estimated time: 10 minutes
\end{itemize}

To complete the experiment in a reasonable amount of time, we perform this
experiment for bitwidths $5$ through $9$ (same as the table in the supplementary
material).

\begin{lstlisting}[mathescape=false, numbers=none, xleftmargin=0cm]
$ cd ../precision-increasing-bitwidth
$ bash pres_inc_bw.sh  
\end{lstlisting}

\emph{Expected Results.} This experiment should output a table which is the same
as Table \ref{table:muls_precision_increasing_bitwidth} in the supplementary
material. It should indicate that the precision of \ourmul as compared to
\kernmul increases, as the bitwidth of the input tnum increases.

\emph{Experiment customization.} The binary corresponding to the source file
\code{precision_increasing_bitwidth.cpp} file accepts a \code{bitwidth} as a
command line option. This allows running the experiment for arbitrary bitwidths
upto $64$. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Methodology}

% Submission, reviewing and badging methodology:

% \begin{itemize}
%   \item \url{https://www.acm.org/publications/policies/artifact-review-badging}
%   \item \url{http://cTuning.org/ae/submission-20201122.html}
%   \item \url{http://cTuning.org/ae/reviewing-20201122.html}
% \end{itemize}




==> tex/sec.semantics.tex <==
\section{Semantics of Tristate Numbers}
\label{sec:semantics}
Prior work has analyzed similar abstract domains that track the individual bits
of a variable. Monniaux \etal \cite{monniaux-device-driver-verification} used it
for analyzing unsigned integer computations in device drivers. Min\'e \etal
\cite{mine-bitfield} have formalized the "Bitfield" Domain, and present a
certain class of abstract transfer functions. Similarly, Regher \etal
\cite{regehr-deriving-abstract-transfer} use a bitwise abstract domain to derive
abstract transfer functions corresponding to a processor's ALU operations. We
note that the tnum abstract domain is distinct from these prior works because it
includes computationally efficient algorithms for abstraction ($\alpha$),
abstract multiplication, addition, and subtraction. Additionally, we show that
our concretization and abstraction functions form a Galios connection. 

% \subsection{\todo{Additional list of things to note in this section}} 

% \begin{itemize}
%   \item Tnums abstract domain lattice
%   \item Concrete domain lattice
%   \item Mathematical formulae of $\alpha, \gamma$
%   \item proof of Galios connection in appendix
%   \item for simple ops, an abstract operation is sound if it is a sound
%   composition of sound abstract operators.
%   \item desigining abstract operators is challenging. In this paper, we 
%   the prove the soundness of the existing ones using z3.
%   \item in cases where z3 doesn't complete verification (multipication),
%   we have a new version which is provable, and faster
%   \item Revisit precision using terms from prior static analysis.
% \end{itemize}

We provide a brief background on tristate numbers (tnums) in the Linux
kernel. Then, we (a) formalize the semantics of tnums, (b) specify the
conditions for well-formedness, and (c) design an algorithm to
construct a precise tnum from a set of concrete values.

\subsection{Background on Tnums}

The BPF verifier in the Linux kernel has to identify whether a BPF
program is safe for all possible inputs when it is loaded into the
kernel. A sub-task in this process is to track the set of values that
a given variable will have during concrete executions of the program
for all inputs. Such information has to be computed with each
arithmetic and logic operation over the variable. Effectively, the BPF static
analyzer needs an abstract
domain~\cite{rival2020introduction} to track such information. The
power-set of all possible values is one such abstract domain. Given an
\nbit variable or a register, the variable can have any of the $2^n$
values (\ie when you interpret the value as an unsigned integer) in a
given execution. The static analysis needs to track the set of values
that the variable can take during various executions of the program
with different inputs (\ie it needs to track an element from the
abstract domain of the power-set of $2^n$ values). As the Linux kernel
needs to perform this static analysis of the BPF program whenever a
program has to be loaded, the computation on the abstract domain has
to be efficient.

\input{figures/fig.tnum.tex}

\textbf{Tnums.}  To track the set of values that each variable can
represent, the Linux kernel uses {\em tristate numbers (\ie tnums)} to
reason about uncertainty at the bit-level. An \nbit variable is
represented by an \nbit tnum. Logically, a bit in a tnum can have one
of three values (hence \emph{tristate} number): $0$, $1$, or $\mu$. A
value of $0$ (similarly $1$) indicates that all executions of the
program will have a 0 (similarly 1) in that specific bit. A value of
$\mu$ for a given bit indicates that the specific bit is unknown.

The Linux kernel concretely implements the tristate number with a
tuple $(v, m)$, where both $v$ and $m$ are n-bit unsigned integers.
For a given bit, a 1 in the $m$ field represents the value $\mu$,
which states that the bit is unknown. If the $m$ field is 0, then the
bit represents a 0 or a 1 depending on the $v$ field of the tnum.
Figure~\ref{fig:tnum}(a) provides a set of values represented by a
4-bit tnum, its logical representation, and the specific
implementation used by the Linux kernel. If the $m$ field of a tnum is
0 (all 0's), then the tnum represents a set with a singleton (a
constant value). If the $m$ field is all 1's, then it represents the
set of all possible values for a given n-bit number.

The Linux kernel reports that an element $x$ belongs to the set of
values represented by a tnum $P$ if the bitwise \texttt{and} of $x$
and the negation of $P.m$ is equal to $P.v$ (\ie $x \, \& \, \lnot
(P.m) = P.v$). Beyond membership, the BPF verifier also defines
algorithms that implement operations on tnums, both arithmetic
(addition, subtraction, multiplication) and bit-level (bit shifts,
bitwise \code{and}, \code{or}, \code{exclusive-or}). These operations
operate directly on the abstract values without generating the
concrete set of values represented by them. They are implemented with
bitwise and arithmetic operations for efficiency. The Linux kernel
neither defines the formal semantics of tnums and its operations, nor
quantifies the loss of precision with abstraction, nor provides
algorithms for constructing tnums from a set of values, nor specifies
the correctness of various tnum operations.

\subsection{Semantics of Tnums}
We highlight the properties of tnums, well-formedness conditions,
precision loss inherent in tnums (compared to a power set abstraction),
and our new algorithm for constructing a tnum given a set of concrete
values.

\textbf{Logical and implementation views of tnums.} In the logical
view of tnums, it is an n-bit representation with each bit
representing $0$ or $1$, or $\mu$. The kernel's implementation
of this logical view is as a tuple with
two \nbit unsigned integers $(v, m)$, where $v$ stands for value and
$m$ stands for mask.

Let $P_{l}[k]$ represent the $k^{th}$-bit in the logical view of the
tnum $P$.  The implementation with the tuple $(v,m)$ is defined as
below:

\begin{small}
\begin{align}
\label{eqn_tnumbasic}
\begin{split}
    (P.v[k] = 0 \wedge P.m[k] = 0) \;\; \triangleq \;\;  P_{l}[k] = 0 \\
    (P.v[k] = 1 \wedge P.m[k] = 0) \;\; \triangleq \;\;  P_{l}[k] = 1 \\
    (P.v[k] = 0 \wedge P.m[k] = 1) \;\; \triangleq \;\;  P_{l}[k] = \mu \\
\end{split}
\end{align}
\end{small}

\textbf{Well-formedness of the implementation view of tnums.} In the
logical view, a bit in a tnum can have only three values: $0$, $1$, or
$\mu$. However, a bit in the implementation $(v, m)$ can have 4
possible bit-patterns. When the $\nth{k}$ bit of both $v$ and $m$ is
set to 1, then the tnum represents an empty set. We define the
implementation $(v,m)$ of the tnum to be well-formed when there is no bit
position $k$ where both $\ithbitx{P.v}{k}$ and $\ithbitx{P.m}{k}$ are
set to \code{1}. That is, $v\ \&\ m$ will always evaluate to $0$.

In the implementation view of tnums with \nbit $v$ and $m$, there are
$2^{n} * 2^{n} = 2^{2n}$ possible tnums. However, there are only $3^n$
tnums from the logical view, since each bit in the logical view can
have one of 3 values. Thus, a large fraction of tnums in the
implementation view are not well-formed, \ie only $3^n$ tnums are
well-formed out of $2^{2n}$ possible tnums in the implementation.


\textbf{Membership.} For a concrete value $x$ and tnum $P: (v, m)$, we
say that $x$ is a member of $P$ (\ie $x \in_{\mathbb{T}} P$,  if the
known bits in $P$ exactly match the bits in $x$). 

\begin{small}
\begin{align}
\begin{split}
    \label{eqn_membership}
    x \in_{\mathbb{T}} P  \Longleftrightarrow   \; (x \, \&\ \, \neg{P.m}) =  P.v \\
    x \notin_{\mathbb{T}} P  \Longleftrightarrow   \; (x \, \&\ \, \neg{P.m}) \neq  P.v 
\end{split}
\end{align}
\end{small}

By the definition of a tnum in \eqref{eqn_tnumbasic}, $P.m$ must
contain a 0 in all the bit positions which are meant to be concrete
(known) in $P$, and 1 in all the bit positions which are unknown in
$P$. To determine membership, we only care that the concrete bits in
$x$ match $P$. $(x \, \&\ \, \neg{P.m})$ will propagate all the bits
which are meant to be concrete bits in $P$, and zero-out the remaining
(unknown) bits. For a well-formed tnum, this expression should
evaluate to $P.v$.


\textbf{Representational imprecision.}  Let $S$ be the set of all
\nbit numbers, then the cardinality (size) of this set, $|S|$, is
$2^n$. If the powerset of all \nbit numbers \ie the set of all
possible subsets of $S$ is $\mathcal{P}(S)$, then the cardinality of
the powerset, $|\mathcal{P}(S)|$ is $2^{2^n}$.  Although there are
$2^{2^{n}}$ possible sets of values, tnums can only represent $3^n$ of
them. Hence, several sets of numbers cannot be represented accurately
using tnums. That is, the tnum representation itself introduces some
imprecision. We call this the {\em representational imprecision.}  For
example, \Fig{tnum}(c) demonstrates that the set $\{1,2\}$ is not
representable precisely with a 4-bit tnum. The smallest superset of
$\{1,2\}$ that can be precisely represented is $\{0,1,2,3\}$, encoded
by the logical tnum $00\mu\mu$.


\textbf{Soundness of tnum operations.} Given a tnum operation
$\texttt{op}_{\mathbb{T}}$ on two tnums $P$ and $Q$ that produces a
result tnum $R$, the operation is sound if the result of the concrete
operation on the values belonging to $P$ and $Q$ is a member of the
set of values represented by $R$.  For any two concrete values, $x
\tnumin P$ and $y \tnumin Q$, the result ($z$) of the concrete
operation on $x$ and $y$ (\ie $z = op_{\mathbb{C}} (x,y)$) is a member
of the set of values represented by tnum $R$ (\ie $z \tnumin R$).

\begin{small}
\begin{align}
\begin{split}
\label{eqn_soundness}
\forall_{P, Q}, 
\forall_{(x \in_{\mathbb{T}} P), (y \in_{\mathbb{T}} Q)}, (z =
\texttt{op}_{\mathbb{C}}(x, y)) \wedge & (R =
\texttt{op}_{\mathbb{T}}(P, Q)) \\ & \implies z \in_{\mathbb{T}} R
\end{split}
\end{align}
\end{small}
  
\textbf{Maximal operational precision for tnum operations.} Apart from the
representational imprecision, a tnum operation itself can introduce
some loss of precision. We say that a tnum operation is {\em maximally
operationally precise} under the following condition. Given two tnums
$P$ and $Q$, if $R$ is the result
of the tnum operation, and if the $\nth{i}$-bit in the result is
unknown (\ie $\ithbitx{R}{i} = \mu$), then there exist concrete values
belonging to the operand tnums (\ie $\{x_{1}, x_{2}\} \tnumin P$
and $\{y_{1}, y_{2}\} \tnumin Q$) such that the result of the
concrete operations on these values differ in the $\nth{i}$-bit.

\begin{small}
\begin{align}
\begin{split}
\label{eqn_precision}
\forall_{P,Q}, & R = \opT (P, Q) \land \ithbitx{R}{i} = \mu \implies \\ 
            & \exists_{(\{x_{1}, x_{2} \} \tnumin {P}) (\{y_{1}, y_{2}\} \tnumin {Q})}, z_{1} = \opC(x_{1}, y_{1}) \; \land \\ 
            & z_{2} = \opC(x_{2}, y_{2}) \land \ithbitx{z_1}{i} \neq \ithbitx{z_2}{i}
\end{split}
\end{align}
\end{small}
 
\subsection{Constructing a Tnum from a Set of Concrete Values}
\label{semantics:shared-bits-tnum}
We present an algorithm to construct a tnum from a set of
concrete values. Let $C$ represent the set of concrete values. From
the definition of tnums, if the $\nth{k}$-bit of all concrete values
in the set are identical, then the bit is a known bit in the
corresponding tnum $P$. Otherwise, the $\nth{k}$-bit of tnum $P$ is unknown.
\begin{small}
\begin{align}
\label{eqn_abs1}
\begin{split}
\forall_{x_{i} \in C}, \ithbitx{x_{i}}{k} = 0 \;  & \longrightarrow \; \ithbitx{P}{k} = 0 \\
\forall_{x_{i} \in C}, \ithbitx{x_{i}}{k} = 1 \;  & \longrightarrow \; \ithbitx{P}{k} = 1 \\
\exists_{x_{i}, x_{j} \in C}, \ithbitx{x_{i}}{k} \neq \ithbitx{x_{j}}{k} \; & \longrightarrow \; \ithbitx{P}{k} = \mu \\
\end{split}
\end{align}
\end{small}

We present a method to construct a tnum implementation $(v,m)$
satisfying the above properties given a concrete set of values.
Figure~\ref{fig:tnum}(c) illustrates our method with an example. Let
$\alpha_{and}$ be the bitwise \texttt{and} of all concrete values in
$C$ (\ie $\alpha_{and} = x_{1}\,\&\,x_{2}\,\&\,x_{3}\,\&\dots$) and
$\alpha_{or}$ be the bitwise \texttt{or} of all concrete values in $C$
(\ie $\alpha_{or} = x_{1}\,|\,x_{2}\,|\,x_{3}\,|\,\dots$). Then, the
tnum implemented by the tuple $(v,m) \triangleq (\alpha_{and}$,
$\alpha_{and} \oplus \alpha_{or})$ contains all the concrete values in
$C$, where $\oplus$ is the bitwise \texttt{exclusive-or} operation.
Appendix~\ref{shared-bits-proof} provides a proof that this algorithm
is sound (\ie the tnum contains all values $x_i \in C$) and is the
most representationally precise tnum for the set $C$.

